A Model-Driven Automation Pipeline for Building Operation

Building Control Systems (BCS) engineering in the Architecture, Engineering, Construction & Operations (AECO) domain remains a complex, manual, and error-prone process, with fractured tools and manual commissioning causing design and built reality to diverge into a performance gap. We argue that a fully integrated and automated, tool-supported workflow spanning design, programming, and operation is feasible and can improve efficiency while reducing manual effort and configuration errors. Building on model-driven engineering, we present an automated process pipeline for modeling, programming, and auto-commissioning BCS. It uses two domain-specific modeling languages with tooling support to synthesize and deploy executable artifacts from platform-independent models, replacing a fractured, multi-stakeholder handoff process with a defined four-step workflow and improving consistency across the engineering lifecycle. Our evaluation reports notable efficiency gains, improved adaptability, moderate-to-high user acceptance, and good performance with solid scalability.

==> fmt.tex <==
\usepackage{fancyhdr}
\usepackage{amsthm}%
\usepackage{mathrsfs}%
\usepackage[title]{appendix}%
\usepackage{manyfoot}%
\usepackage{algorithm}%
\usepackage{algorithmicx}%
\usepackage{algpseudocode}%
\usepackage{listings}%
\usepackage{amsmath,amssymb,amsfonts} %%assymb breaks the acm template
\usepackage{url}
\usepackage{booktabs} % For formal tables                  
%\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
%\usepackage{xcolor}
\usepackage{xspace}
\usepackage{hyperref}
\usepackage{balance}
\usepackage{tabularx}

\usepackage{booktabs}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{caption}
%\usepackage{subfigure}
\usepackage{subcaption}
\usepackage[export]{adjustbox}
\usepackage{tabularx}
\usepackage{tikz}
\usepackage{float}
\usepackage[shortlabels]{enumitem}
\usepackage[font=small]{caption}

\usepackage{csquotes}
\MakeOuterQuote{"}




%\usepackage{xcolor}
\usepackage{url}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{array}
\usepackage{color}
\usepackage{wasysym}
\usepackage{verbatim}
\usepackage{bigstrut}
\usepackage{multirow}
%\usepackage{amsmath}
\usepackage{setspace}
\usepackage{tabularx}
\usepackage{url}
\usepackage{xspace}
\usepackage{pifont}
\usepackage{subcaption}
\usepackage[font=footnotesize]{caption}%,labelfont=bf]{caption}
\usepackage{array,booktabs}
\usepackage{soul}
\usepackage{vcell}
\usepackage{pifont}
\usepackage{afterpage}
\usepackage{rotating}
\usepackage{wrapfig}
\usepackage{caption}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{enumitem}
\usepackage{lipsum}
%\usepackage{xcolor}
\usepackage{balance}
\usepackage{tikz}
\usepackage{hyperref}
\usepackage{tabularx}
\usepackage{booktabs}














\definecolor{commentGreen}{RGB}{128,127,41}
\definecolor{stringGreen}{RGB}{0,127,38}
\definecolor{keywordRed}{RGB}{151,0,11}
\definecolor{typePurple}{RGB}{128,3,82}
\definecolor{variableBlue}{RGB}{0,0,255}
\definecolor{annotationRed}{RGB}{198,4,38}
\definecolor{annotationBlue}{RGB}{32,21,223}

\newcommand{\etal}{\emph{et~al.}\xspace}

\newcommand{\citesec}[1]{Section~\ref{sec:#1}}
\newcommand{\citefig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\citealgo}[1]{\textsc{Listing}~\ref{algo:#1}}
\newcommand{\citelisting}[1]{\textsc{Listing}~\ref{lst:#1}}
\newcommand{\citetable}[1]{{Table}~\ref{tab:#1}}
\newcommand{\citedef}[1]{\textsc{Definition}~\ref{def:#1}}
\newcommand{\citesecs}[2]{Sections~\ref{sec:#1} and~\ref{sec:#2}}

% \newcommand{\mv}[1]{{\textcolor{orange}{#1}}}%orange
% \newcommand{\ig}[1]{{\textcolor{blue}{#1}}}%blue
% \newcommand{\ta}[1]{{\textcolor{green}{#1}}}%green

% \newcommand{\fwname}{{\textcolor{purple} EduComp}\xspace}%orange


\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash}p{#1}} 


\newcommand{\bullitem}[1]{\noindent$\bullet$\textbf{ #1}}

\newcommand{\intqte}[1]{\emph{#1}}


\newcommand{\archname}{{SoS-PuDZ}\xspace}
\newcommand{\pubtop}[1]{{\texttt{\small #1}\xspace}}



\newcommand{\MtoH}{\textbf{$[M \rightarrow H]$}\xspace}
\newcommand{\HtoM}{\textbf{$[H \rightarrow M]$}\xspace}

\newcommand{\jch}[1]{{\textcolor{blue}{#1}}} %blue
\newcommand{\ankit}[1]{{\textcolor{purple}{#1}}} %purple
\newcommand{\mv}[1]{{\textcolor{orange}{#1}}}%orange
\newcommand{\mkhmt}{{\it MAPE-K$_{HMT}$}\xspace}
\newcommand{\DR}{{\it Drone Response}\xspace}
\newcommand{\DRx}{{\it Drone Response}}
\newcommand{\pudz}{{\it PuDZ}\xspace}


\newcommand{\ttformat}[1]{{\texttt{\small #1}}}

\definecolor{alizarin}{rgb}{0.82, 0.1, 0.26}
\newcommand{\hlt}[1]{{\textcolor{alizarin}{#1}}}%orange
\newcommand{\markphase}{ \CIRCLE}
\hyphenation{autono-mous}


